Restricted Permutations Enumerated by Inversions

Permutations are usually enumerated by size, but new results can be found by enumerating them by inversions instead, in which case one must restrict one's attention to indecomposable permutations. In the style of the seminal paper by Simion and Schmidt, we investigate all combinations of permutation patterns of length at most 3.

==> eptcsdata.tex <==
\providecommand{\firstpage}{96}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2024\\
EPTCS 403, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.403.21}{10.4204/EPTCS.403.21}}

